Combining Constraint Programming Reasoning with Large Language Model Predictions

Constraint Programming (CP) and Machine Learning (ML) face challenges in text generation due to CP's struggle with implementing "meaning'' and ML's difficulty with structural constraints. This paper proposes a solution by combining both approaches and embedding a Large Language Model (LLM) in CP. The LLM handles word generation and meaning, while CP manages structural constraints. This approach builds on GenCP, an improved version of On-the-fly Constraint Programming Search (OTFS) using LLM-generated domains. Compared to Beam Search (BS), a standard NLP method, this combined approach (GenCP with LLM) is faster and produces better results, ensuring all constraints are satisfied. This fusion of CP and ML presents new possibilities for enhancing text generation under constraints.

==> 0_results/arrays/CPvBSwSpace.tex <==
\begin{table}[htbp]
    \resizebox{0.5\textwidth}{!}{
        \begin{tabular}{*{7}{|c}||*{3}{c|}}
        % \begin{tabular}{*{5}{|p{1.5cm}}||*{3}{p{1.5cm}|}}
            \cline{1-10}
            % \multicolumn{1}{c}{} & \multicolumn{7}{|c||}{Time (seconds)} & \multicolumn{7}{c|}{Space (megabytes)}\\
            % \hline
            % \N & \T& Temps CPU (s) & \# Backtrack & \# Nœuds & Temps CPU (s) & \# Backtrack & \# Nœuds & \# Appels utiles & \# Appels inutiles\\
            \multicolumn{3}{|c|}{Experiments} & \multicolumn{4}{|c||}{BS} & \multicolumn{3}{c|}{\otf}\\
            \hline
            sent & k & \#sols & (s) & (mb) & \#badoutput & \%sat & (s) & (mb) & \#bk\\
            \hline

                        
                        
            1 & 5 & 1 & 108 & 7 & 9 & 10\% & 103 & 5 & 45\\
             \hline
             & 10 & 0 & 182 & 13 & 18 & 0\% &177 & 10 & 84\\
             \hline
             & 20 & 1 & 399 & 36 & 58 &1\%& 46 & 4 & 13\\
             \hline
             & 50 & 1 & 1123 & 131 & 109 & $\approx 0\%$ & 47 & 7 & 13\\
            \hline
            \hline
            2 & 5 & 5 & 34 & 3 & 0 & 100\% &  38 & 1 & 38\\
             \hline
             & 10 & 10 & 69 & 7 & 0 &100\% & 36 & 5 & 25\\
             \hline
             & 20 & 20 & 140 & 22 & 0 &100\% & 58 & 9 & 40\\
             \hline
             & 50 & 49 & 354 & 75 & 1 & 99\% & 134 & 24 & 100\\
            \hline
            \hline
            3 & 5 & 0 & 248 & 12 & 5 & 0\% & 36 & 2 & 4\\
             \hline
             & 10 & 2 & 510 & 29 & 8 & 20\% & 55 & 3 & 6\\
             \hline
             & 20 & 4 & 1030 & 73 & 16 & 20\% & 164 & 8 & 38\\
             \hline
             & 50 & 20 & 2633 & 244 & 30 & 66\% & 1174 & 67 & 374\\
            \hline
            \hline
            4 & 5 & 25 & 279 & 23 & 3 & 89\%& 308 & 13 & 118\\
             \hline
             & 10 & 30 & 513 & 72 & 8 & 78\%  & 311 & 16 & 114\\
             \hline
             & 20 & 45 & 1123 & 180 & 14 & 76\% & 321 & 19 & 104\\
             \hline
             & 50 & 89 & 2928 & 785 & 40 & 68\% & 388 & 19 & 27\\
            \hline
        \end{tabular}
    }
    \caption{Comparison of BeamSearch and our approach on different tasks.
    }\label{er:arrcpvbswspace}
\end{table}

==> 0_results/arrays/arrExp1-4.tex <==
% ajouter colonnes "output" pour BS
% afin d'ajouter colones %sat (pourcentages de sols/output) de constraintes.
% ajouter col #bk
\begin{table}[htbp]
    \resizebox{0.5\textwidth}{!}{
        \begin{tabular}{*{7}{|c}||*{3}{c|}}
        % \begin{tabular}{*{5}{|p{1.5cm}}||*{3}{p{1.5cm}|}}
            \cline{1-9}
            % \multicolumn{1}{c}{} & \multicolumn{7}{|c||}{Time (seconds)} & \multicolumn{7}{c|}{Space (megabytes)}\\
            % \hline
            % \N & \T& Temps CPU (s) & \# Backtrack & \# Nœuds & Temps CPU (s) & \# Backtrack & \# Nœuds & \# Appels utiles & \# Appels inutiles\\
            \multicolumn{3}{|c|}{Experiments} & \multicolumn{4}{|c||}{BS} & \multicolumn{3}{c|}{\otf}\\
            \hline
            sent & k & \#sols & (s) & (mb) & \#badoutput & \%sat & (s) & (mb) & \#bk\\
            \hline
            %1 & 5 & 5 & 127 & 19 & 5 & 50\% & 42 & 5 & 11\\
            % \hline
            %1 & 10 & 4 & 255 & 31 & 10& 28\% & 31 & 2 & 6\\
            % \hline
            %1 & 20 & 11 & 526 & 74 & 18 & 37\% & 55 & 4 & 13\\
            % \hline
            %1 & 50 & 32 & 1276 & 274 & 41 & 43\% & 141 & 12 & 41\\
            % \hline
             %\hline
            %2 & 5 & 1 & 249 & 15 & 4 & 20\%  &42 & 3 & 10\\
             %\hline
            %2 & 10 & 0 & 425 & 55 & 10 & 0\% & 54 & 3 & 12\\
             %\hline
            %2 & 20 & 14 & 974 & 153 & 18 & 63\%& 170 & 12 & 49\\
             %\hline
            %2 & 50 & 9 & 2459 & 688 & 50 & 15\% & 117 & 10 & 30\\
             %\hline
             \hline
            3 & 5 & 1 & 108 & 7 & 9 & 10\% & 103 & 5 & 45\\
             \hline
            3 & 10 & 0 & 182 & 13 & 18 & 0\% &177 & 10 & 84\\
             \hline
            3 & 20 & 1 & 399 & 36 & 58 &1\%& 46 & 4 & 13\\
             \hline
            3 & 50 & 1 & 1123 & 131 & 109 & \approx 0\% & 47 & 7 & 13\\
            \hline
            \hline
            4 & 5 & 5 & 34 & 3 & 0 & 100\% &  38 & 1 & 38\\
             \hline
            4 & 10 & 10 & 69 & 7 & 0 &100\% & 36 & 5 & 25\\
             \hline
            4 & 20 & 20 & 140 & 22 & 0 &100\% & 58 & 9 & 40\\
             \hline
            4 & 50 & 49 & 354 & 75 & 1 & 99\% & 134 & 24 & 100\\
            \hline
        \end{tabular}
    }
    \caption{Comparison of BeamSearch and our approach on different tasks.
    }\label{er:arr14}
\end{table}


 %sent-1& $\in [12,16]$ &  & is that a                \\
     %sent-2& $\in [18,22]$ &  & John, car seller, BMW \\
     %sent-3&     & $=82$ &  \\
     %sent-4& $=10$    &  & $X_3 =$ soft, $X_7 =$ soft,$X_{10} =$ math  \\
     
     %sent-5& $\geq 20$   & $\forall i, |X_i| \le 6$ &   \\
    % sent-6&    &   & a, e, t as forbidden letters    \\
     %sent-7&    &   & soft, beach, math   \\
     % \hline
    % sent-8&    & $\in [110,140]$, $\forall i, |X_i| \geq 4$  & beam search, constraint programming\\
     % & & & u is a forbidden letter\\

==> 0_results/arrays/arrExp5-8.tex <==
\begin{table}[htbp]
    \resizebox{0.5\textwidth}{!}{
    
        \begin{tabular}{*{7}{|c}||*{3}{c|}}
            \cline{1-9}
            \multicolumn{3}{|c|}{Experiments} & \multicolumn{4}{|c||}{BS} & \multicolumn{3}{c|}{\otf}\\
            \hline
            sent & k & \#sols & time(s) & space(mb) & \#output & \%sat & time(s) & space(mb) & \#bk\\
            \hline
            5 & 5 & 0 & 248 & 12 & 5 & 0\% & 36 & 2 & 4\\
             \hline
            5 & 10 & 2 & 510 & 29 & 8 & 20\% & 55 & 3 & 6\\
             \hline
            5 & 20 & 4 & 1030 & 73 & 16 & 20\% & 164 & 8 & 38\\
             \hline
            5 & 50 & 20 & 2633 & 244 & 30 & 66\% & 1174 & 67 & 374\\
            % \hline
            % \hline
           % 6 & 5 & 0 & 108 & 9 & 5 & 0\% & 41 & 3 & 13\\
            % \hline
           % 6 & 10 & 3 & 225 & 25 & 7 & 33\% & 49 & 4 & 13\\
             %\hline
           % 6 & 20 & 4 & 452 & 74 & 16 & 20\% & 53 & 5 & 13\\
             %\hline
           % 6 & 50 & 20 & 1180 & 276 & 22 & 47\% & 141 & 12 & 13\\
             \hline
             \hline
            7 & 5 & 25 & 279 & 23 & 3 & 89\% & 308 & 13 & 118\\
             \hline
            7 & 10 & 30 & 513 & 72 & 8 & 78\%  & 311 & 16 & 114\\
             \hline
            7 & 20 & 45 & 1123 & 180 & 14 & 76\% & 321 & 19 & 104\\
             \hline
            7 & 50 & 89 & 2928 & 785 & 40 & 68\% & 388 & 19 & 27\\
            \hline
            %\hline
            %8 & 5 & 2 & 273 & 17 & 5 & 28\% & 25 & 2 & 3\\
            % \hline
            %8 & 10 & 10 & 569 & 42 & 10 & 50\% & 113 & 7 & 30\\
            % \hline
            %8 & 20 & 15 & 1150 & 109 & 20 & 42\%  & 168 & 14 & 50\\
             %\hline
            %8 & 50 & 49 & 2170 & 443 & 50 & 49\% & 432 & 39 & 110\\
            %\hline
        \end{tabular}
    }
    \caption{Comparison of BeamSearch and our approach on different tasks.
    }\label{er:arr58}
\end{table}
 %sent-1& $\in [12,16]$ &  & is that a                \\
     %sent-2& $\in [18,22]$ &  & John, car seller, BMW \\
     %sent-3&     & $=82$ &  \\
     %sent-4& $=10$    &  & $X_3 =$ soft, $X_7 =$ soft,$X_{10} =$ math  \\
     
     %sent-5& $\geq 20$   & $\forall i, |X_i| \le 6$ &   \\
    % sent-6&    &   & a, e, t as forbidden letters    \\
     %sent-7&    &   & soft, beach, math   \\
     % \hline
    % sent-8&    & $\in [110,140]$, $\forall i, |X_i| \geq 4$  & beam search, constraint programming\\
     % & & & u is a forbidden letter\\

==> 0_results/arrays/arrResSentence.tex <==
\begin{table}[htbp]
    \resizebox{0.5\textwidth}{!}{
        \begin{tabular}{*{4}{|c}|}
        % \begin{tabular}{*{5}{|p{1.5cm}}||*{3}{p{1.5cm}|}}
            \cline{1-4}
            % \multicolumn{1}{c}{} & \multicolumn{7}{|c||}{Time (seconds)} & \multicolumn{7}{c|}{Space (megabytes)}\\
            % \hline
            % \N & \T& Temps CPU (s) & \# Backtrack & \# Nœuds & Temps CPU (s) & \# Backtrack & \# Nœuds & \# Appels utiles & \# Appels inutiles\\
            % \multicolumn{1}{c}{} & \multicolumn{1}{c}{Experiment number} & \multicolumn{1}{c}{k} & \multicolumn{1}{c|}{Sentences generated}\\
             & n & k & Sentences generated\\
            \hline
            BS & 1 & 5 & The following is that a your mom.\\
            \hline
            \otf & 1 & 5 & The following is that a your dad.\\
            \hline
        \end{tabular}
    }
    \caption{Sample of sentence generated by beamsearch and our approach.
    }\label{er:arrSen}
\end{table}


==> 0_results/arrays/arrResStats.tex <==
\begin{table*}[htbp]
    \resizebox{\textwidth}{!}{
        \begin{tabular}{*{7}{|c}||*{5}{c|}}
        % \begin{tabular}{*{5}{|p{1.5cm}}||*{3}{p{1.5cm}|}}
            \cline{1-12}
            % \multicolumn{1}{c}{} & \multicolumn{7}{|c||}{Time (seconds)} & \multicolumn{7}{c|}{Space (megabytes)}\\
            % \hline
            % \N & \T& Temps CPU (s) & \# Backtrack & \# Nœuds & Temps CPU (s) & \# Backtrack & \# Nœuds & \# Appels utiles & \# Appels inutiles\\
            \multicolumn{2}{|c|}{Experiment} & \multicolumn{5}{|c||}{Beam Search} & \multicolumn{5}{c|}{Our Approach}\\
            \hline
            number & k & time(s) & space(mb) & \#sol & \#sol valid & var & time(s) & space(mb) & \#sol & \#sol valid & var\\
            \hline
            1 & 10 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
            1 & 20 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
            2 & 10 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
            2 & 20 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
            3 & 10 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
            3 & 20 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
            4 & 10 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
            4 & 20 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
            5 & 10 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
            5 & 20 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100\\
             \hline
        \end{tabular}
    }
    \caption{Comparison of BeamSearch and our approach on different problems.
    }\label{er:arrStat}
\end{table*}


==> inc/textGeneration.tex <==

%\section{Text Generation with constraints}
%\label{sec:TextGen}

%\flo{Introduire la problematique de la generation de texte ici, que c'est tres rechercher, qu'est ce que notre papier apporte à ce domaine ? Introduire beam search et les benchs ici}
